Investigating the translation capabilities of Large Language Models trained on parallel data only

In recent years, Large Language Models (LLMs) have demonstrated exceptional proficiency across a broad spectrum of Natural Language Processing (NLP) tasks, including Machine Translation. However, previous methods predominantly relied on iterative processes such as instruction fine-tuning or continual pre-training, leaving unexplored the challenges of training LLMs solely on parallel data. In this work, we introduce PLUME (Parallel Language Model), a collection of three 2B LLMs featuring varying vocabulary sizes (32k, 128k, and 256k) trained exclusively on Catalan-centric parallel examples. These models perform comparably to previous encoder-decoder architectures on 16 supervised translation directions and 56 zero-shot ones. Utilizing this set of models, we conduct a thorough investigation into the translation capabilities of LLMs, probing their performance, the impact of the different elements of the prompt, and their cross-lingual representation space.

==> figures/attention_matrix/attention_figure2.tex <==
\begin{figure}[!b]
  \centering
  \begin{tikzpicture}
    \draw[step=0.4cm,gray,very thin] (0,0) grid (4,4);
    \draw (0,0) -- (4,0) -- (4,4) -- (0,4) -- cycle;

    % Masked future tokens
    \foreach \x/\y in {0.4/3.6, 0.8/3.2, 1.2/2.8, 1.6/2.4, 2.0/2.0, 2.4/1.6, 2.8/1.2, 3.2/0.8, 3.6/0.4} {
      \fill[blue!40!white] (\x,\y) rectangle (4, \y+0.4);
    }

    % BOS Attention
    \fill[red!40!white] (0.0,0.0) rectangle (0.4,4);

    % Source tag attention
    \fill[green!40!white] (0.4,0.0) rectangle (0.8,3.6);

    % Cross attention
    \fill[yellow!40!white] (0.8,0.0) rectangle (2.4,1.6);

    % Target tag attention
    \fill[orange!40!white] (2.4,0.0) rectangle (2.8,1.6);
    
  \end{tikzpicture}
  \caption{} % Add caption text if needed
  \label{fig:masked_sa}
\end{figure}
